Nuclear modification factor of neutral pions in the forward and backward regions in $p$-Pb collisions

The nuclear modification factor of neutral pions is measured in proton-lead collisions collected at a center-of-mass energy per nucleon of $8.16~{\rm TeV}$ with the LHCb detector. The $\pi^0$ production cross section is measured differentially in transverse momentum ($p_{\rm T}$) for $1.5<p_{\rm T}<10.0~{\rm GeV}$ and in center-of-mass pseudorapidity ($\eta_{\rm c.m.}$) regions $2.5<\eta_{\rm c.m.}<3.5$ (forward) and $-4.0<\eta_{\rm c.m.}<-3.0$ (backward) defined relative to the proton beam direction. The forward measurement shows a sizable suppression of $\pi^0$ production, while the backward measurement shows the first evidence of $\pi^0$ enhancement in proton-lead collisions at the LHC. Together, these measurements provide precise constraints on models of nuclear structure and particle production in high-energy nuclear collisions.

==> Authorship_LHCb-PAPER-2021-053.tex <==
% LHCb collaboration author list
% Data extracted on June 1st, 2023 at 12:58pm for paper reference LHCb-PAPER-2021-053
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{50}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{44}$,
F.~Abudin{\'e}n$^{50}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{54}$\lhcborcid{0000-0002-5951-3498},
B.~Adeva$^{40}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{48}$\lhcborcid{0000-0002-1326-1264},
H.~Afsharnia$^{9}$,
C.~Agapopoulou$^{13}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{77}$\lhcborcid{0000-0001-9540-4988},
S.~Aiola$^{25}$\lhcborcid{0000-0001-6209-7627},
Z.~Ajaltouni$^{9}$,
S.~Akar$^{59}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{32}$\lhcborcid{0000-0002-6736-471X},
J.~Albrecht$^{15}$\lhcborcid{0000-0001-8636-1621},
F.~Alessio$^{42}$\lhcborcid{0000-0001-5317-1098},
M.~Alexander$^{53}$\lhcborcid{0000-0002-8148-2392},
A.~Alfonso~Albero$^{39}$\lhcborcid{0000-0001-6025-0675},
Z.~Aliouche$^{56}$\lhcborcid{0000-0003-0897-4160},
P.~Alvarez~Cartelle$^{49}$\lhcborcid{0000-0003-1652-2834},
S.~Amato$^{2}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{48}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{11}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{42}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{22}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{44}$\lhcborcid{0000-0003-3594-9163},
A.~Andreianov$^{38}$\lhcborcid{0000-0002-6273-0506},
M.~Andreotti$^{21}$\lhcborcid{0000-0003-2918-1311},
D.~Ao$^{6}$\lhcborcid{0000-0003-1647-4238},
F.~Archilli$^{17}$\lhcborcid{0000-0002-1779-6813},
A.~Artamonov$^{38}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{62}$\lhcborcid{0000-0002-5991-7273},
K.~Arzymatov$^{38}$,
E.~Aslanides$^{10}$\lhcborcid{0000-0003-3286-683X},
M.~Atzeni$^{44}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
S.~Bachmann$^{17}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{43}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{50}$\lhcborcid{0000-0001-7791-4490},
A.~Bailly-reyre$^{13}$,
P.~Baladron~Rodriguez$^{40}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{12}$\lhcborcid{0000-0002-1611-7188},
W.~Baldini$^{21}$\lhcborcid{0000-0001-7658-8777},
J.~Baptista~de~Souza~Leite$^{1}$\lhcborcid{0000-0002-4442-5372},
M.~Barbetti$^{22,j}$\lhcborcid{0000-0002-6704-6914},
R.J.~Barlow$^{56}$\lhcborcid{0000-0002-8295-8612},
S.~Barsuk$^{11}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{55}$\lhcborcid{0000-0002-9264-4799},
M.~Bartolini$^{49}$\lhcborcid{0000-0002-8479-5802},
F.~Baryshnikov$^{38}$\lhcborcid{0000-0002-6418-6428},
J.M.~Basels$^{14}$\lhcborcid{0000-0001-5860-8770},
G.~Bassi$^{29,q}$\lhcborcid{0000-0002-2145-3805},
B.~Batsukh$^{4}$\lhcborcid{0000-0003-1020-2549},
A.~Battig$^{15}$\lhcborcid{0009-0001-6252-960X},
A.~Bay$^{43}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{50}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{15}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{29}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{1}$\lhcborcid{0000-0001-7806-5283},
A.~Beiter$^{62}$,
V.~Belavin$^{38}$,
S.~Belin$^{40}$\lhcborcid{0000-0001-7154-1304},
V.~Bellee$^{44}$\lhcborcid{0000-0001-5314-0953},
K.~Belous$^{38}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{38}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{38}$\lhcborcid{0000-0002-7458-7030},
G.~Bencivenni$^{23}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{13}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{38}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{44}$\lhcborcid{0000-0002-4856-8063},
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{62}$,
C.~Bertella$^{56}$\lhcborcid{0000-0002-3160-147X},
A.~Bertolin$^{28}$\lhcborcid{0000-0003-1393-4315},
C.~Betancourt$^{44}$\lhcborcid{0000-0001-9886-7427},
F.~Betti$^{42}$\lhcborcid{0000-0002-2395-235X},
Ia.~Bezshyiko$^{44}$\lhcborcid{0000-0002-4315-6414},
S.~Bhasin$^{48}$\lhcborcid{0000-0002-0146-0717},
J.~Bhom$^{35}$\lhcborcid{0000-0002-9709-903X},
L.~Bian$^{67}$\lhcborcid{0000-0001-5209-5097},
M.S.~Bieker$^{15}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{21}$\lhcborcid{0000-0003-3004-0946},
S.~Bifani$^{47}$\lhcborcid{0000-0001-7072-4854},
P.~Billoir$^{13}$\lhcborcid{0000-0001-5433-9876},
A.~Biolchini$^{32}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{55}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{49}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{56}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{}$\lhcborcid{0000-0001-5729-5530},
M.~Bj{\o}rn$^{57}$,
M.P.~Blago$^{49}$\lhcborcid{0000-0001-7542-2388},
T.~Blake$^{50}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{43}$\lhcborcid{0000-0001-5775-3132},
S.~Blusk$^{62}$\lhcborcid{0000-0001-9170-684X},
D.~Bobulska$^{53}$\lhcborcid{0000-0002-3003-9980},
J.A.~Boelhauve$^{15}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{40}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{59}$\lhcborcid{0000-0002-2439-9955},
A.~Boldyrev$^{38}$\lhcborcid{0000-0002-7872-6819},
N.~Bondar$^{38,42}$\lhcborcid{0000-0003-2714-9879},
S.~Borghi$^{56}$\lhcborcid{0000-0001-5135-1511},
M.~Borisyak$^{38}$,
M.~Borsato$^{17}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{35}$\lhcborcid{0000-0002-9065-9030},
S.A.~Bouchiba$^{43}$\lhcborcid{0000-0002-0044-6470},
T.J.V.~Bowcock$^{54,42}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{42}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{21}$\lhcborcid{0000-0001-6782-3982},
M.J.~Bradley$^{55}$,
S.~Braun$^{60}$\lhcborcid{0000-0002-4489-1314},
A.~Brea~Rodriguez$^{40}$\lhcborcid{0000-0001-5650-445X},
J.~Brodzicka$^{35}$\lhcborcid{0000-0002-8556-0597},
A.~Brossa~Gonzalo$^{50}$\lhcborcid{0000-0002-4442-1048},
D.~Brundu$^{27}$\lhcborcid{0000-0003-4457-5896},
A.~Buonaura$^{44}$\lhcborcid{0000-0003-4907-6463},
L.~Buonincontri$^{28}$\lhcborcid{0000-0002-1480-454X},
A.T.~Burke$^{56}$\lhcborcid{0000-0003-0243-0517},
C.~Burr$^{42}$\lhcborcid{0000-0002-5155-1094},
A.~Bursche$^{66}$,
A.~Butkevich$^{38}$\lhcborcid{0000-0001-9542-1411},
J.S.~Butter$^{32}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{42}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{42}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{27}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{67}$,
R.~Calabrese$^{21,i}$\lhcborcid{0000-0002-1354-5400},
L.~Calefice$^{15,13}$\lhcborcid{0000-0001-6401-1583},
S.~Cali$^{23}$\lhcborcid{0000-0001-9056-0711},
R.~Calladine$^{47}$,
M.~Calvi$^{26,m}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{75}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{48}$\lhcborcid{0000-0003-3641-8110},
P.~Campana$^{23}$\lhcborcid{0000-0001-8233-1951},
D.H.~Campora~Perez$^{74}$\lhcborcid{0000-0001-8998-9975},
A.F.~Campoverde~Quezada$^{6}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{26,m}$\lhcborcid{0000-0002-8444-4498},
L.~Capriotti$^{20,g}$\lhcborcid{0000-0003-4899-0587},
A.~Carbone$^{20,g}$\lhcborcid{0000-0002-7045-2243},
G.~Carboni$^{31}$\lhcborcid{0000-0003-1128-8276},
R.~Cardinale$^{24,k}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{27}$\lhcborcid{0000-0002-6649-0298},
I.~Carli$^{4}$\lhcborcid{0000-0002-0411-1141},
P.~Carniti$^{26,m}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{14}$,
A.~Casais~Vidal$^{40}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{17}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{54}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{42}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{42}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{21,i}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{43}$\lhcborcid{0000-0003-4715-7622},
J.~Cerasoli$^{10}$\lhcborcid{0000-0001-9777-881X},
D.~Cervenkov$^{57}$\lhcborcid{0000-0002-1865-741X},
A.J.~Chadwick$^{54}$\lhcborcid{0000-0003-3537-9404},
M.G.~Chapman$^{48}$,
M.~Charles$^{13}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{42}$\lhcborcid{0000-0001-9295-8635},
C.A.~Chavez~Barajas$^{54}$\lhcborcid{0000-0002-4602-8661},
M.~Chefdeville$^{8}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{3}$\lhcborcid{0000-0002-3400-5489},
S.~Chen$^{4}$\lhcborcid{0000-0002-8647-1828},
A.~Chernov$^{35}$\lhcborcid{0000-0003-0232-6808},
V.~Chobanova$^{40}$\lhcborcid{0000-0002-1353-6002},
S.~Cholak$^{43}$\lhcborcid{0000-0001-8091-4766},
M.~Chrzaszcz$^{35}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{38}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{38}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{23}$\lhcborcid{0000-0003-0253-9846},
M.F.~Cicala$^{50}$\lhcborcid{0000-0003-0678-5809},
X.~Cid~Vidal$^{40}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{42}$\lhcborcid{0000-0003-1002-8368},
G.~Ciullo$^{i,21}$\lhcborcid{0000-0001-8297-2206},
P.E.L.~Clarke$^{52}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{42}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{49}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{42}$\lhcborcid{0000-0002-0228-9130},
J.L.~Cobbledick$^{56}$\lhcborcid{0000-0002-5146-9605},
V.~Coco$^{42}$\lhcborcid{0000-0002-5310-6808},
J.A.B.~Coelho$^{11}$\lhcborcid{0000-0001-5615-3899},
J.~Cogan$^{10}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{9}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{37}$\lhcborcid{0000-0002-1281-5923},
P.~Collins$^{42}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{42}$\lhcborcid{0000-0002-9617-9687},
L.~Congedo$^{19,f}$\lhcborcid{0000-0003-4536-4644},
A.~Contu$^{27}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{47}$\lhcborcid{0000-0002-4179-3700},
G.~Coombs$^{53}$\lhcborcid{0000-0003-4621-2757},
I.~Corredoira~$^{40}$\lhcborcid{0000-0002-6089-0899},
G.~Corti$^{42}$\lhcborcid{0000-0003-2857-4471},
C.M.~Costa~Sobral$^{50}$\lhcborcid{0000-0002-3899-4894},
B.~Couturier$^{42}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{58}$\lhcborcid{0000-0002-3684-1560},
J.~Crkovsk\'{a}$^{61}$\lhcborcid{0000-0002-7946-7580},
M.~Cruz~Torres$^{1,e}$\lhcborcid{0000-0003-2607-131X},
R.~Currie$^{52}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{61}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{38}$\lhcborcid{0000-0002-0093-3244},
L.~Dai$^{65}$\lhcborcid{0000-0002-4070-4729},
E.~Dall'Occo$^{15}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{40}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{42}$\lhcborcid{0000-0003-4344-9994},
A.~Danilina$^{38}$\lhcborcid{0000-0003-3121-2164},
P.~d'Argent$^{42}$\lhcborcid{0000-0003-2380-8355},
J.E.~Davies$^{56}$\lhcborcid{0000-0002-5382-8683},
A.~Davis$^{56}$\lhcborcid{0000-0001-9458-5115},
O.~De~Aguiar~Francisco$^{56}$\lhcborcid{0000-0003-2735-678X},
J.~de~Boer$^{42}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{73}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{56}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{43}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{1}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{23}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{1}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{2}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{19,f}$\lhcborcid{0000-0003-4915-7933},
D.~De~Simone$^{44}$\lhcborcid{0000-0001-8180-4366},
P.~De~Simone$^{23}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{15}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{74}$\lhcborcid{0000-0003-4712-9816},
C.T.~Dean$^{61}$\lhcborcid{0000-0002-6002-5870},
F.~Debernardis$^{19,f}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{8}$\lhcborcid{0000-0001-9643-6762},
V.~Dedu$^{10}$\lhcborcid{0000-0001-5672-8672},
L.~Del~Buono$^{13}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{49}$\lhcborcid{0009-0007-6371-8035},
H.-P.~Dembinski$^{15}$\lhcborcid{0000-0003-3337-3850},
V.~Denysenko$^{44}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{9}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{27,h}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{71}$\lhcborcid{0000-0002-4563-5806},
A.~Di~Cicco$^{23}$\lhcborcid{0000-0002-6925-8056},
P.~Di~Nezza$^{23}$\lhcborcid{0000-0003-4894-6762},
S.~Didenko$^{38}$\lhcborcid{0000-0001-5671-5863},
L.~Dieste~Maronas$^{40}$,
S.~Ding$^{62}$\lhcborcid{0000-0002-5946-581X},
V.~Dobishuk$^{46}$\lhcborcid{0000-0001-9004-3255},
C.~Dong$^{3}$\lhcborcid{0000-0003-3259-6323},
A.M.~Donohoe$^{18}$\lhcborcid{0000-0002-4438-3950},
F.~Dordei$^{27}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{1}$\lhcborcid{0000-0001-7517-8418},
L.~Douglas$^{53}$,
A.G.~Downes$^{8}$\lhcborcid{0000-0003-0217-762X},
M.W.~Dudek$^{35}$\lhcborcid{0000-0003-3939-3262},
L.~Dufour$^{42}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{72}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{42}$\lhcborcid{0000-0002-1204-2270},
J.M.~Durham$^{61}$\lhcborcid{0000-0002-5831-3398},
D.~Dutta$^{56}$\lhcborcid{0000-0002-1191-3978},
A.~Dziurda$^{35}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{38}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{51}$\lhcborcid{0000-0002-4027-7333},
U.~Egede$^{63}$\lhcborcid{0000-0001-5493-0762},
V.~Egorychev$^{38}$\lhcborcid{0000-0002-2539-673X},
S.~Eidelman$^{38,\dagger}$,
S.~Eisenhardt$^{52}$\lhcborcid{0000-0002-4860-6779},
S.~Ek-In$^{43}$\lhcborcid{0000-0002-2232-6760},
L.~Eklund$^{76}$\lhcborcid{0000-0002-2014-3864},
S.~Ely$^{62}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{37}$\lhcborcid{0000-0001-5513-0927},
E.~Epple$^{61}$\lhcborcid{0000-0002-6312-3740},
S.~Escher$^{14}$\lhcborcid{0009-0007-2540-4203},
J.~Eschle$^{44}$\lhcborcid{0000-0002-7312-3699},
S.~Esen$^{44}$\lhcborcid{0000-0003-2437-8078},
T.~Evans$^{56}$\lhcborcid{0000-0003-3016-1879},
L.N.~Falcao$^{1}$\lhcborcid{0000-0003-3441-583X},
Y.~Fan$^{6}$\lhcborcid{0000-0002-3153-430X},
B.~Fang$^{67}$\lhcborcid{0000-0003-0030-3813},
S.~Farry$^{54}$\lhcborcid{0000-0001-5119-9740},
D.~Fazzini$^{26,m}$\lhcborcid{0000-0002-5938-4286},
M.~Feo$^{42}$\lhcborcid{0000-0001-5266-2442},
A.~Fernandez~Prieto$^{40}$\lhcborcid{0000-0003-1984-6367},
A.D.~Fernez$^{60}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{20}$\lhcborcid{0000-0002-3721-4585},
L.~Ferreira~Lopes$^{43}$\lhcborcid{0009-0003-5290-823X},
F.~Ferreira~Rodrigues$^{2}$\lhcborcid{0000-0002-4274-5583},
S.~Ferreres~Sole$^{32}$\lhcborcid{0000-0003-3571-7741},
M.~Ferrillo$^{44}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{42}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{38}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{19}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{21,i}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{34}$\lhcborcid{0000-0002-1084-0084},
K.M.~Fischer$^{57}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{77}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{56}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{34}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{12}$\lhcborcid{0000-0002-2430-782X},
M.~Fontana$^{13}$\lhcborcid{0000-0003-4727-831X},
F.~Fontanelli$^{24,k}$\lhcborcid{0000-0001-7029-7178},
R.~Forty$^{42}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{49}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{54}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{60}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{42}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{21,i}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{17}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{42}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{53}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{6}$\lhcborcid{0000-0003-3177-2700},
Q.~Fuehring$^{15}$\lhcborcid{0000-0003-3179-2525},
E.~Gabriel$^{32}$\lhcborcid{0000-0001-8300-5939},
G.~Galati$^{19,f}$\lhcborcid{0000-0001-7348-3312},
A.~Gallas~Torreira$^{40}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{20,g}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{52,42}$\lhcborcid{0000-0003-2420-0501},
Y.~Gan$^{3}$\lhcborcid{0009-0006-6576-9293},
M.~Gandelman$^{2}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{25}$\lhcborcid{0000-0001-7267-6008},
Y.~Gao$^{5}$\lhcborcid{0000-0003-1484-0943},
M.~Garau$^{27,h}$\lhcborcid{0000-0002-0505-9584},
L.M.~Garcia~Martin$^{50}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{39}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,m}$\lhcborcid{0000-0003-2316-8829},
B.~Garcia~Plana$^{40}$,
F.A.~Garcia~Rosales$^{12}$\lhcborcid{0000-0003-4395-0244},
L.~Garrido$^{39}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{42}$\lhcborcid{0000-0002-8009-1509},
R.E.~Geertsema$^{32}$\lhcborcid{0000-0001-6829-7777},
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{56}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{56}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{50}$\lhcborcid{0000-0002-3183-5065},
L.~Giambastiani$^{28}$\lhcborcid{0000-0002-5170-0635},
V.~Gibson$^{49}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{36}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{57}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{23,t}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{40}$\lhcborcid{0000-0001-5399-326X},
P.~Gironella~Gironell$^{39}$\lhcborcid{0000-0001-5603-4750},
C.~Giugliano$^{21,i}$\lhcborcid{0000-0002-6159-4557},
K.~Gizdov$^{52}$\lhcborcid{0000-0002-3543-7451},
E.L.~Gkougkousis$^{42}$\lhcborcid{0000-0002-2132-2071},
V.V.~Gligorov$^{13,42}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{64}$\lhcborcid{0000-0003-0523-495X},
E.~Golobardes$^{75}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{38}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{55,38}$\lhcborcid{0000-0003-2500-8247},
A.~Gomes$^{1,a}$\lhcborcid{0009-0005-2892-2968},
S.~Gomez~Fernandez$^{39}$\lhcborcid{0000-0002-3064-9834},
F.~Goncalves~Abrantes$^{57}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{35}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{3}$\lhcborcid{0000-0002-7822-3947},
I.V.~Gorelov$^{38}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{26}$\lhcborcid{0000-0003-2501-9608},
J.P.~Grabowski$^{17}$\lhcborcid{0000-0001-8461-8382},
T.~Grammatico$^{13}$\lhcborcid{0000-0002-2818-9744},
L.A.~Granado~Cardoso$^{42}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{39}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{43}$\lhcborcid{0000-0003-4647-6429},
G.~Graziani$^{}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{37}$\lhcborcid{0000-0002-7770-1839},
L.M.~Greeven$^{32}$\lhcborcid{0000-0001-5813-7972},
N.A.~Grieser$^{4}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{56}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{38}$\lhcborcid{0000-0002-8967-3644},
B.R.~Gruberg~Cazon$^{57}$\lhcborcid{0000-0003-4313-3121},
C. ~Gu$^{3}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{21,i}$\lhcborcid{0000-0001-8829-9681},
M.~Guittiere$^{11}$\lhcborcid{0000-0002-2916-7184},
P. A.~G{\"u}nther$^{17}$\lhcborcid{0000-0002-4057-4274},
E.~Gushchin$^{38}$\lhcborcid{0000-0001-8857-1665},
A.~Guth$^{14}$,
Y.~Guz$^{38}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{42}$\lhcborcid{0000-0002-6825-6497},
T.~Hadavizadeh$^{63}$\lhcborcid{0000-0001-5730-8434},
G.~Haefeli$^{43}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{42}$\lhcborcid{0000-0002-4947-2928},
J.~Haimberger$^{42}$\lhcborcid{0000-0002-3363-7783},
S.C.~Haines$^{49}$\lhcborcid{0000-0001-5906-391X},
T.~Halewood-leagas$^{54}$\lhcborcid{0000-0001-9629-7029},
M.M.~Halvorsen$^{42}$\lhcborcid{0000-0003-0959-3853},
P.M.~Hamilton$^{60}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{54}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{7}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{17}$\lhcborcid{0000-0001-7641-7505},
E.B.~Hansen$^{56}$\lhcborcid{0000-0002-5019-1648},
S.~Hansmann-Menzemer$^{17,42}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{6}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{57}$\lhcborcid{0000-0001-9616-6651},
T.~Harrison$^{54}$\lhcborcid{0000-0002-1576-9205},
C.~Hasse$^{42}$\lhcborcid{0000-0002-9658-8827},
M.~Hatch$^{42}$\lhcborcid{0009-0004-4850-7465},
J.~He$^{6,c}$\lhcborcid{0000-0002-1465-0077},
K.~Heijhoff$^{32}$\lhcborcid{0000-0001-5407-7466},
K.~Heinicke$^{15}$\lhcborcid{0009-0003-8781-3425},
R.D.L.~Henderson$^{63,50}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{58}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{54}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{42}$\lhcborcid{0000-0003-3605-832X},
J.~Heuel$^{14}$\lhcborcid{0000-0001-9384-6926},
A.~Hicheur$^{2}$\lhcborcid{0000-0002-3712-7318},
D.~Hill$^{43}$\lhcborcid{0000-0003-2613-7315},
M.~Hilton$^{56}$\lhcborcid{0000-0001-7703-7424},
S.E.~Hollitt$^{15}$\lhcborcid{0000-0002-4962-3546},
R.~Hou$^{7}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{8}$\lhcborcid{0000-0001-6454-278X},
J.~Hu$^{17}$,
J.~Hu$^{66}$\lhcborcid{0000-0002-8227-4544},
W.~Hu$^{7}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{3}$\lhcborcid{0000-0002-5924-2683},
W.~Huang$^{6}$\lhcborcid{0000-0002-1407-1729},
X.~Huang$^{67}$,
W.~Hulsbergen$^{32}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{50}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{38}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{54}$\lhcborcid{0000-0002-4174-6509},
D.~Hynds$^{32}$\lhcborcid{0009-0009-0976-2312},
P.~Ibis$^{15}$\lhcborcid{0000-0002-2022-6862},
M.~Idzik$^{34}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{38}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{59}$\lhcborcid{0000-0001-5534-1732},
A.~Inglessi$^{38}$\lhcborcid{0000-0002-2522-6722},
A.~Iniukhin$^{38}$\lhcborcid{0000-0002-1940-6276},
A.~Ishteev$^{38}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{38}$\lhcborcid{0000-0001-8403-0706},
R.~Jacobsson$^{42}$\lhcborcid{0000-0003-4971-7160},
H.~Jage$^{14}$\lhcborcid{0000-0002-8096-3792},
S.~Jakobsen$^{42}$\lhcborcid{0000-0002-6564-040X},
E.~Jans$^{32}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{41}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{60}$\lhcborcid{0000-0003-3719-119X},
V.~Jevtic$^{15}$\lhcborcid{0000-0001-6427-4746},
X.~Jiang$^{4,6}$\lhcborcid{0000-0001-8120-3296},
M.~John$^{57}$\lhcborcid{0000-0002-8579-844X},
D.~Johnson$^{58}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{49}$\lhcborcid{0000-0003-1699-8816},
T.P.~Jones$^{50}$\lhcborcid{0000-0001-5706-7255},
B.~Jost$^{42}$\lhcborcid{0009-0005-4053-1222},
N.~Jurik$^{42}$\lhcborcid{0000-0002-6066-7232},
S.~Kandybei$^{45}$\lhcborcid{0000-0003-3598-0427},
Y.~Kang$^{3}$\lhcborcid{0000-0002-6528-8178},
M.~Karacson$^{42}$\lhcborcid{0009-0006-1867-9674},
D.~Karpenkov$^{38}$\lhcborcid{0000-0001-8686-2303},
M.~Karpov$^{38}$\lhcborcid{0000-0003-4503-2682},
J.W.~Kautz$^{59}$\lhcborcid{0000-0001-8482-5576},
F.~Keizer$^{42}$\lhcborcid{0000-0002-1290-6737},
D.M.~Keller$^{62}$\lhcborcid{0000-0002-2608-1270},
M.~Kenzie$^{50}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{33}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{15}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{38}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{38}$\lhcborcid{0000-0002-0260-6570},
T.~Kirn$^{14}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{43}$\lhcborcid{0009-0005-4421-9025},
O.~Kitouni$^{58}$\lhcborcid{0000-0001-9695-8165},
S.~Klaver$^{33}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{29,q}$\lhcborcid{0000-0003-0828-0943},
K.~Klimaszewski$^{36}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{36}$\lhcborcid{0000-0002-1821-1848},
S.~Koliiev$^{46}$\lhcborcid{0009-0002-3680-1224},
A.~Kondybayeva$^{38}$\lhcborcid{0000-0001-8727-6840},
A.~Konoplyannikov$^{38}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{34}$\lhcborcid{0000-0001-9092-3527},
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$\lhcborcid{0000-0001-8614-7203},
M.~Korolev$^{38}$\lhcborcid{0000-0002-7473-2031},
I.~Kostiuk$^{32,46}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{46}$,
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
A.~Kozachuk$^{38}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{38}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{38}$\lhcborcid{0000-0001-8631-4200},
R.D.~Krawczyk$^{42}$\lhcborcid{0000-0001-8664-4787},
M.~Kreps$^{50}$\lhcborcid{0000-0002-6133-486X},
S.~Kretzschmar$^{14}$\lhcborcid{0009-0008-8631-9552},
P.~Krokovny$^{38}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{34}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{36}$\lhcborcid{0000-0002-9546-358X},
J.~Kubat$^{17}$,
W.~Kucewicz$^{35,34}$\lhcborcid{0000-0002-2073-711X},
M.~Kucharczyk$^{35}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{38}$\lhcborcid{0009-0000-2192-995X},
H.S.~Kuindersma$^{32}$,
G.J.~Kunde$^{61}$,
T.~Kvaratskheliya$^{38}$,
D.~Lacarrere$^{42}$\lhcborcid{0009-0005-6974-140X},
G.~Lafferty$^{56}$\lhcborcid{0000-0003-0658-4919},
A.~Lai$^{27}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{27,h}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{44}$\lhcborcid{0000-0003-1587-4555},
J.J.~Lane$^{56}$\lhcborcid{0000-0002-5816-9488},
R.~Lane$^{48}$\lhcborcid{0000-0002-2360-2392},
G.~Lanfranchi$^{23}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{14}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{15}$\lhcborcid{0000-0002-0322-5550},
O.~Lantwin$^{38}$\lhcborcid{0000-0003-2384-5973},
T.~Latham$^{50}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{29,u}$\lhcborcid{0000-0002-3151-3453},
M.~Lazzaroni$^{25,l}$\lhcborcid{0000-0002-4094-1273},
R.~Le~Gac$^{10}$\lhcborcid{0000-0002-7551-6971},
S.H.~Lee$^{77}$\lhcborcid{0000-0003-3523-9479},
R.~Lef{\`e}vre$^{9}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{38}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{38}$\lhcborcid{0000-0003-3192-6175},
P.~Lenisa$^{i,21}$\lhcborcid{0000-0003-3509-1240},
O.~Leroy$^{10}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{35}$\lhcborcid{0000-0002-3966-2998},
B.~Leverington$^{17}$\lhcborcid{0000-0001-6640-7274},
H.~Li$^{66}$\lhcborcid{0000-0002-2366-9554},
P.~Li$^{17}$\lhcborcid{0000-0003-2740-9765},
S.~Li$^{7}$\lhcborcid{0000-0001-5455-3768},
Y.~Li$^{4}$\lhcborcid{0000-0003-2043-4669},
Z.~Li$^{62}$\lhcborcid{0000-0003-0755-8413},
X.~Liang$^{62}$\lhcborcid{0000-0002-5277-9103},
T.~Lin$^{55}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{42}$\lhcborcid{0000-0002-5541-6500},
V.~Lisovskyi$^{15}$\lhcborcid{0000-0003-4451-214X},
R.~Litvinov$^{27,h}$\lhcborcid{0000-0002-4234-435X},
G.~Liu$^{66}$\lhcborcid{0000-0001-5961-6588},
H.~Liu$^{6}$\lhcborcid{0000-0001-6658-1993},
Q.~Liu$^{6}$\lhcborcid{0000-0003-4658-6361},
S.~Liu$^{4,6}$\lhcborcid{0000-0002-6919-227X},
A.~Lobo~Salvia$^{39}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{27}$\lhcborcid{0000-0003-4176-1503},
R.~Lollini$^{72}$\lhcborcid{0000-0003-3898-7464},
J.~Lomba~Castro$^{40}$\lhcborcid{0000-0003-1874-8407},
I.~Longstaff$^{53}$,
J.H.~Lopes$^{2}$\lhcborcid{0000-0003-1168-9547},
S.~L{\'o}pez~Soli{\~n}o$^{40}$\lhcborcid{0000-0001-9892-5113},
G.H.~Lovell$^{49}$\lhcborcid{0000-0002-9433-054X},
Y.~Lu$^{4,b}$\lhcborcid{0000-0003-4416-6961},
C.~Lucarelli$^{22,j}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{28,o}$\lhcborcid{0000-0003-4937-7637},
S.~Luchuk$^{38}$\lhcborcid{0000-0002-3697-8129},
M.~Lucio~Martinez$^{32}$\lhcborcid{0000-0001-6823-2607},
V.~Lukashenko$^{32,46}$\lhcborcid{0000-0002-0630-5185},
Y.~Luo$^{3}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{56}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{21,i}$\lhcborcid{0000-0002-1072-5633},
O.~Lupton$^{50}$\lhcborcid{0000-0002-3500-7398},
A.~Lusiani$^{29,q}$\lhcborcid{0000-0002-6876-3288},
X.-R.~Lyu$^{6}$\lhcborcid{0000-0001-5689-9578},
L.~Ma$^{4}$\lhcborcid{0009-0004-5695-8274},
R.~Ma$^{6}$\lhcborcid{0000-0002-0152-2412},
S.~Maccolini$^{20}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{11}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{37}$\lhcborcid{0000-0001-6651-9436},
V.~Macko$^{43}$\lhcborcid{0009-0003-8228-0404},
P.~Mackowiak$^{15}$\lhcborcid{0009-0007-6216-7155},
S.~Maddrell-Mander$^{48}$,
L.R.~Madhan~Mohan$^{48}$\lhcborcid{0000-0002-9390-8821},
A.~Maevskiy$^{38}$\lhcborcid{0000-0003-1652-8005},
D.~Maisuzenko$^{38}$\lhcborcid{0000-0001-5704-3499},
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{57}$\lhcborcid{0000-0002-8179-0707},
B.~Malecki$^{35}$\lhcborcid{0000-0003-0062-1985},
A.~Malinin$^{38}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{38}$\lhcborcid{0000-0002-2120-5633},
H.~Malygina$^{17}$\lhcborcid{0000-0002-1807-3430},
G.~Manca$^{27,h}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{10}$\lhcborcid{0000-0003-1144-3678},
D.~Manuzzi$^{20}$\lhcborcid{0000-0002-9915-6587},
C.A.~Manzari$^{44}$\lhcborcid{0000-0001-8114-3078},
D.~Marangotto$^{25,l}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{8}$\lhcborcid{0000-0002-4111-0797},
U.~Marconi$^{20}$\lhcborcid{0000-0002-5055-7224},
S.~Mariani$^{22,j}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{42}$\lhcborcid{0000-0003-0529-6982},
M.~Marinangeli$^{43}$\lhcborcid{0000-0002-8361-9356},
J.~Marks$^{17}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{48}$\lhcborcid{0000-0002-9863-4954},
P.J.~Marshall$^{54}$,
G.~Martelli$^{72,p}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{30}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{42,m}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{26,m}$\lhcborcid{0000-0003-4792-9178},
D.~Martinez~Santos$^{40}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{41}$\lhcborcid{0000-0001-6841-6035},
A.~Massafferri$^{1}$\lhcborcid{0000-0002-3264-3401},
M.~Materok$^{14}$\lhcborcid{0000-0002-7380-6190},
R.~Matev$^{42}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{44}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{38}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{26}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{77}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{32}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{12}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{39}$\lhcborcid{0000-0002-9331-1363},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
M.~McCann$^{55}$\lhcborcid{0000-0002-3038-7301},
L.~Mcconnell$^{18}$\lhcborcid{0009-0004-7045-2181},
T.H.~McGrath$^{56}$\lhcborcid{0000-0001-8993-3234},
N.T.~McHugh$^{53}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{56}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{18}$\lhcborcid{0000-0001-7144-0175},
J.V.~Mead$^{54}$\lhcborcid{0000-0003-0875-2533},
B.~Meadows$^{59}$\lhcborcid{0000-0002-1947-8034},
G.~Meier$^{15}$\lhcborcid{0000-0002-4266-1726},
D.~Melnychuk$^{36}$\lhcborcid{0000-0003-1667-7115},
S.~Meloni$^{26,m}$\lhcborcid{0000-0003-1836-0189},
M.~Merk$^{32,74}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{25,l}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{2}$\lhcborcid{0000-0002-2622-8551},
M.~Mikhasenko$^{69,d}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{68}$\lhcborcid{0000-0001-7450-1121},
E.~Millard$^{50}$,
M.~Milovanovic$^{42}$\lhcborcid{0000-0003-1580-0898},
M.-N.~Minard$^{8,\dagger}$,
A.~Minotti$^{26,m}$\lhcborcid{0000-0002-0091-5177},
S.E.~Mitchell$^{52}$\lhcborcid{0000-0002-7956-054X},
B.~Mitreska$^{56}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{15}$\lhcborcid{0000-0003-3650-2689},
A.~M{\"o}dden~$^{15}$\lhcborcid{0009-0009-9185-4901},
R.A.~Mohammed$^{57}$\lhcborcid{0000-0002-3718-4144},
R.D.~Moise$^{55}$\lhcborcid{0000-0002-5662-8804},
S.~Mokhnenko$^{38}$\lhcborcid{0000-0002-1849-1472},
T.~Momb{\"a}cher$^{40}$\lhcborcid{0000-0002-5612-979X},
I.A.~Monroy$^{68}$\lhcborcid{0000-0001-8742-0531},
S.~Monteil$^{9}$\lhcborcid{0000-0001-5015-3353},
M.~Morandin$^{28}$\lhcborcid{0000-0003-4708-4240},
G.~Morello$^{23}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{29,q}$\lhcborcid{0000-0003-4190-1078},
J.~Moron$^{34}$\lhcborcid{0000-0002-1857-1675},
A.B.~Morris$^{69}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{50}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{62}$\lhcborcid{0000-0003-1908-4219},
H.~Mu$^{3}$\lhcborcid{0000-0001-9720-7507},
F.~Muheim$^{52}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{73}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{44}$\lhcborcid{0000-0002-5105-1305},
C.H.~Murphy$^{57}$\lhcborcid{0000-0002-6441-075X},
D.~Murray$^{56}$\lhcborcid{0000-0002-5729-8675},
R.~Murta$^{55}$\lhcborcid{0000-0002-6915-8370},
P.~Muzzetto$^{27,h}$\lhcborcid{0000-0003-3109-3695},
P.~Naik$^{48}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{43}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{51}$\lhcborcid{0000-0002-6813-6794},
T.~Nanut$^{42}$\lhcborcid{0000-0002-5728-9867},
I.~Nasteva$^{2}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{52}$\lhcborcid{0000-0002-8297-6714},
N.~Neri$^{25,l}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{69}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{42}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{38}$,
R.~Newcombe$^{55}$,
E.M.~Niel$^{43}$\lhcborcid{0000-0002-6587-4695},
S.~Nieswand$^{14}$,
N.~Nikitin$^{38}$\lhcborcid{0000-0003-0215-1091},
N.S.~Nolte$^{58}$\lhcborcid{0000-0003-2536-4209},
C.~Normand$^{8,h,27}$\lhcborcid{0000-0001-5055-7710},
C.~Nunez$^{77}$\lhcborcid{0000-0002-2521-9346},
A.~Oblakowska-Mucha$^{34}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{38}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{14}$\lhcborcid{0000-0001-7792-4082},
D.P.~O'Hanlon$^{48}$\lhcborcid{0000-0002-3001-6690},
S.~Okamura$^{21,i}$\lhcborcid{0000-0003-1229-3093},
R.~Oldeman$^{27,h}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{52}$\lhcborcid{0000-0001-7025-3407},
M.E.~Olivares$^{62}$,
C.J.G.~Onderwater$^{73}$\lhcborcid{0000-0002-2310-4166},
R.H.~O'Neil$^{52}$\lhcborcid{0000-0002-9797-8464},
J.M.~Otalora~Goicochea$^{2}$\lhcborcid{0000-0002-9584-8500},
T.~Ovsiannikova$^{38}$\lhcborcid{0000-0002-3890-9426},
P.~Owen$^{44}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{41}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{52}$\lhcborcid{0000-0003-3227-9248},
K.O.~Padeken$^{69}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{50}$\lhcborcid{0000-0003-3184-1622},
P.R.~Pais$^{42}$\lhcborcid{0009-0005-9758-742X},
T.~Pajero$^{57}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{19}$\lhcborcid{0000-0002-6095-9593},
M.~Palutan$^{23}$\lhcborcid{0000-0001-7052-1360},
Y.~Pan$^{56}$\lhcborcid{0000-0002-4110-7299},
G.~Panshin$^{38}$\lhcborcid{0000-0001-9163-2051},
A.~Papanestis$^{51}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{19,f}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{21,i}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{59}$\lhcborcid{0000-0003-0738-3668},
W.~Parker$^{60}$\lhcborcid{0000-0001-9479-1285},
C.~Parkes$^{56}$\lhcborcid{0000-0003-4174-1334},
B.~Passalacqua$^{21,i}$\lhcborcid{0000-0003-3643-7469},
G.~Passaleva$^{22}$\lhcborcid{0000-0002-8077-8378},
A.~Pastore$^{19}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{55}$\lhcborcid{0000-0003-3871-5602},
C.~Patrignani$^{20,g}$\lhcborcid{0000-0002-5882-1747},
C.J.~Pawley$^{74}$\lhcborcid{0000-0001-9112-3724},
A.~Pearce$^{42}$\lhcborcid{0000-0002-9719-1522},
A.~Pellegrino$^{32}$\lhcborcid{0000-0002-7884-345X},
M.~Pepe~Altarelli$^{42}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{20}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{38}$\lhcborcid{0000-0002-7008-8082},
A.~Pereiro~Castro$^{40}$\lhcborcid{0000-0001-9721-3325},
P.~Perret$^{9}$\lhcborcid{0000-0002-5732-4343},
M.~Petric$^{53}$,
K.~Petridis$^{48}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{24,k}$\lhcborcid{0000-0003-0222-7594},
A.~Petrov$^{38}$,
S.~Petrucci$^{52}$\lhcborcid{0000-0001-8312-4268},
M.~Petruzzo$^{25}$\lhcborcid{0000-0001-8377-149X},
H.~Pham$^{62}$\lhcborcid{0000-0003-2995-1953},
A.~Philippov$^{38}$\lhcborcid{0000-0002-5103-8880},
R.~Piandani$^{6}$\lhcborcid{0000-0003-2226-8924},
L.~Pica$^{29,q}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{72}$\lhcborcid{0000-0001-8659-4409},
B.~Pietrzyk$^{8}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{11}$\lhcborcid{0000-0001-9622-820X},
M.~Pili$^{57}$\lhcborcid{0000-0002-7599-4666},
D.~Pinci$^{30}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{42}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{26,m,42}$\lhcborcid{0000-0001-5189-230X},
V.~Placinta$^{37}$\lhcborcid{0000-0003-4465-2441},
J.~Plews$^{47}$\lhcborcid{0009-0009-8213-7265},
M.~Plo~Casasus$^{40}$\lhcborcid{0000-0002-2289-918X},
F.~Polci$^{13,42}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{23}$\lhcborcid{0000-0001-7867-1232},
M.~Poliakova$^{62}$,
A.~Poluektov$^{10}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{38}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{62}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{2}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{42}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{6,42}$\lhcborcid{0000-0002-8293-2922},
S.~Popov$^{38}$\lhcborcid{0000-0003-2849-3233},
S.~Poslavskii$^{38}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{35}$\lhcborcid{0000-0001-9923-0938},
L.~Promberger$^{42}$\lhcborcid{0000-0003-0127-6255},
C.~Prouve$^{40}$\lhcborcid{0000-0003-2000-6306},
V.~Pugatch$^{46}$\lhcborcid{0000-0002-5204-9821},
V.~Puill$^{11}$\lhcborcid{0000-0003-0806-7149},
G.~Punzi$^{29,r}$\lhcborcid{0000-0002-8346-9052},
H.R.~Qi$^{3}$\lhcborcid{0000-0002-9325-2308},
W.~Qian$^{6}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{3}$\lhcborcid{0000-0001-8453-658X},
R.~Quagliani$^{43}$\lhcborcid{0000-0002-3632-2453},
N.V.~Raab$^{18}$\lhcborcid{0000-0002-3199-2968},
R.I.~Rabadan~Trejo$^{6}$\lhcborcid{0000-0002-9787-3910},
B.~Rachwal$^{34}$\lhcborcid{0000-0002-0685-6497},
J.H.~Rademacker$^{48}$\lhcborcid{0000-0003-2599-7209},
R.~Rajagopalan$^{62}$,
M.~Rama$^{29}$\lhcborcid{0000-0003-3002-4719},
M.~Ramos~Pernas$^{50}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{2}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{38}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{33,42}$\lhcborcid{0000-0002-2897-5323},
M.~Reboud$^{8}$\lhcborcid{0000-0001-6033-3606},
F.~Redi$^{42}$\lhcborcid{0000-0001-9728-8984},
F.~Reiss$^{56}$\lhcborcid{0000-0002-8395-7654},
C.~Remon~Alepuz$^{41}$,
Z.~Ren$^{3}$\lhcborcid{0000-0001-9974-9350},
V.~Renaudin$^{57}$\lhcborcid{0000-0003-4440-937X},
P.K.~Resmi$^{10}$\lhcborcid{0000-0001-9025-2225},
R.~Ribatti$^{29,q}$\lhcborcid{0000-0003-1778-1213},
A.M.~Ricci$^{27}$\lhcborcid{0000-0002-8816-3626},
S.~Ricciardi$^{51}$\lhcborcid{0000-0002-4254-3658},
K.~Rinnert$^{54}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{11}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{52}$\lhcborcid{0000-0002-7026-1383},
A.B.~Rodrigues$^{43}$\lhcborcid{0000-0002-1955-7541},
E.~Rodrigues$^{54}$\lhcborcid{0000-0003-2846-7625},
J.A.~Rodriguez~Lopez$^{68}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{40}$\lhcborcid{0000-0002-7973-8061},
A.~Rollings$^{57}$\lhcborcid{0000-0002-5213-3783},
P.~Roloff$^{42}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{38}$\lhcborcid{0000-0003-0939-4272},
M.~Romero~Lamas$^{40}$\lhcborcid{0000-0002-1217-8418},
A.~Romero~Vidal$^{40}$\lhcborcid{0000-0002-8830-1486},
J.D.~Roth$^{77,\dagger}$,
M.~Rotondo$^{23}$\lhcborcid{0000-0001-5704-6163},
M.S.~Rudolph$^{62}$\lhcborcid{0000-0002-0050-575X},
T.~Ruf$^{42}$\lhcborcid{0000-0002-8657-3576},
R.A.~Ruiz~Fernandez$^{40}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{41}$,
A.~Ryzhikov$^{38}$\lhcborcid{0000-0002-3543-0313},
J.~Ryzka$^{34}$\lhcborcid{0000-0003-4235-2445},
J.J.~Saborido~Silva$^{40}$\lhcborcid{0000-0002-6270-130X},
N.~Sagidova$^{38}$\lhcborcid{0000-0002-2640-3794},
N.~Sahoo$^{47}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{27,h}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{42}$\lhcborcid{0009-0007-9229-653X},
C.~Sanchez~Gras$^{32}$\lhcborcid{0000-0002-7082-887X},
I.~Sanderswood$^{41}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{30}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{40}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{23}$\lhcborcid{0000-0002-8776-6759},
E.~Santovetti$^{31,t}$\lhcborcid{0000-0002-5605-1662},
D.~Saranin$^{38}$\lhcborcid{0000-0002-9617-9986},
G.~Sarpis$^{14}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{69}$\lhcborcid{0000-0002-6402-1674},
A.~Sarti$^{30}$\lhcborcid{0000-0001-5419-7951},
C.~Satriano$^{30,s}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{31}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{15}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{38}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{9}$\lhcborcid{0000-0003-2689-1123},
L.G.~Scantlebury~Smead$^{57}$\lhcborcid{0000-0001-8702-7991},
A.~Scarabotto$^{13}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{14}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{54}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{53}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{42}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{16}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{42}$\lhcborcid{0000-0002-8400-1566},
S.~Schmitt$^{14}$\lhcborcid{0000-0002-6394-1081},
O.~Schneider$^{43}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{42}$\lhcborcid{0000-0002-8581-3312},
M.~Schubiger$^{32}$\lhcborcid{0000-0001-9330-1440},
S.~Schulte$^{43}$\lhcborcid{0009-0001-8533-0783},
M.H.~Schune$^{11}$\lhcborcid{0000-0002-3648-0830},
R.~Schwemmer$^{42}$\lhcborcid{0009-0005-5265-9792},
B.~Sciascia$^{23,42}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{42}$\lhcborcid{0000-0002-8568-1487},
S.~Sellam$^{40}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{38}$\lhcborcid{0000-0003-1130-2197},
M.~Senghi~Soares$^{33}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{24,k}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{44}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{28}$\lhcborcid{0000-0002-1127-5144},
A.~Seuthe$^{15}$\lhcborcid{0000-0002-0736-3061},
Y.~Shang$^{5}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{77}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{38}$\lhcborcid{0000-0002-4098-9592},
I.~Shchemerov$^{38}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{43}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{54}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{38}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{5}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{4,6}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{38}$\lhcborcid{0000-0003-3171-9125},
E.B.~Shields$^{26,m}$\lhcborcid{0000-0001-5836-5211},
Y.~Shimizu$^{11}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{38}$\lhcborcid{0000-0002-8868-1730},
J.D.~Shupperd$^{62}$\lhcborcid{0009-0006-8218-2566},
B.G.~Siddi$^{21,i}$\lhcborcid{0000-0002-3004-187X},
R.~Silva~Coutinho$^{44}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{28}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{19,f}$\lhcborcid{0000-0003-3631-8398},
M.~Singla$^{63}$\lhcborcid{0000-0003-3204-5847},
N.~Skidmore$^{56}$\lhcborcid{0000-0003-3410-0731},
R.~Skuza$^{17}$\lhcborcid{0000-0001-6057-6018},
T.~Skwarnicki$^{62}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{47}$\lhcborcid{0000-0002-2687-1950},
I.~Slazyk$^{21,i}$\lhcborcid{0000-0002-3513-9737},
J.C.~Smallwood$^{57}$\lhcborcid{0000-0003-2460-3327},
J.G.~Smeaton$^{49}$\lhcborcid{0000-0002-8694-2853},
E.~Smith$^{44}$\lhcborcid{0000-0002-9740-0574},
M.~Smith$^{55}$\lhcborcid{0000-0002-3872-1917},
A.~Snoch$^{32}$\lhcborcid{0000-0001-6431-6360},
L.~Soares~Lavra$^{9}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{59}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{53}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{38,48}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{38}$\lhcborcid{0000-0003-4254-6012},
I.~Solovyev$^{38}$\lhcborcid{0000-0003-4254-6012},
F.L.~Souza~De~Almeida$^{2}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{2}$\lhcborcid{0009-0003-3794-3408},
B.~Spaan$^{15,\dagger}$,
E.~Spadaro~Norella$^{25,l}$\lhcborcid{0000-0002-1111-5597},
E.~Spiridenkov$^{38}$,
P.~Spradlin$^{53}$\lhcborcid{0000-0002-5280-9464},
F.~Stagni$^{42}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{59}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{42}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{57}$\lhcborcid{0000-0003-1776-0498},
O.~Steinkamp$^{44}$\lhcborcid{0000-0001-7055-6467},
O.~Stenyakin$^{38}$,
H.~Stevens$^{15}$\lhcborcid{0000-0002-9474-9332},
S.~Stone$^{62,\dagger}$\lhcborcid{0000-0002-2122-771X},
D.~Strekalina$^{38}$\lhcborcid{0000-0003-3830-4889},
F.~Suljik$^{57}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{27}$\lhcborcid{0000-0002-6020-2304},
L.~Sun$^{67}$\lhcborcid{0000-0002-0034-2567},
Y.~Sun$^{60}$\lhcborcid{0000-0003-4933-5058},
P.~Svihra$^{56}$\lhcborcid{0000-0002-7811-2147},
P.N.~Swallow$^{47}$\lhcborcid{0000-0003-2751-8515},
K.~Swientek$^{34}$\lhcborcid{0000-0001-6086-4116},
A.~Szabelski$^{36}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{34}$\lhcborcid{0000-0002-2562-7163},
M.~Szymanski$^{42}$\lhcborcid{0000-0002-9121-6629},
S.~Taneja$^{56}$\lhcborcid{0000-0001-8856-2777},
A.R.~Tanner$^{48}$,
M.D.~Tat$^{57}$\lhcborcid{0000-0002-6866-7085},
A.~Terentev$^{38}$\lhcborcid{0000-0003-2574-8560},
F.~Teubert$^{42}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{42}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{47}$\lhcborcid{0000-0003-1196-5943},
K.A.~Thomson$^{54}$\lhcborcid{0000-0003-3111-4003},
H.~Tilquin$^{55}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{9}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{8}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{4}$\lhcborcid{0000-0002-2047-7020},
L.~Tomassetti$^{21,i}$\lhcborcid{0000-0003-4184-1335},
X.~Tong$^{5}$\lhcborcid{0000-0002-5278-1203},
D.~Torres~Machado$^{1}$\lhcborcid{0000-0001-7030-6468},
D.Y.~Tou$^{3}$\lhcborcid{0000-0002-4732-2408},
E.~Trifonova$^{38}$,
S.M.~Trilov$^{48}$\lhcborcid{0000-0003-0267-6402},
C.~Trippl$^{43}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{6}$\lhcborcid{0000-0002-0364-5758},
A.~Tully$^{43}$\lhcborcid{0000-0002-8712-9055},
N.~Tuning$^{32,42}$\lhcborcid{0000-0003-2611-7840},
A.~Ukleja$^{36}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{17}$\lhcborcid{0000-0002-1484-2546},
E.~Ursov$^{38}$\lhcborcid{0000-0002-6519-4526},
A.~Usachov$^{32}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{38}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{17}$\lhcborcid{0000-0002-8514-3777},
A.~Vagner$^{38}$,
V.~Vagnoni$^{20}$\lhcborcid{0000-0003-2206-311X},
A.~Valassi$^{42}$\lhcborcid{0000-0001-9322-9565},
G.~Valenti$^{20}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{75}$\lhcborcid{0000-0001-8748-8448},
M.~van~Beuzekom$^{32}$\lhcborcid{0000-0002-0500-1286},
M.~Van~Dijk$^{43}$\lhcborcid{0000-0003-2538-5798},
H.~Van~Hecke$^{61}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{38}$\lhcborcid{0000-0001-8807-8811},
M.~van~Veghel$^{73}$\lhcborcid{0000-0001-6178-6623},
R.~Vazquez~Gomez$^{39}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{40}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{42}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{21}$\lhcborcid{0000-0002-4311-3166},
J.J.~Velthuis$^{48}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{22,v}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{62}$\lhcborcid{0000-0001-6950-1477},
M.~Veronesi$^{32}$\lhcborcid{0000-0002-1916-3884},
M.~Vesterinen$^{50}$\lhcborcid{0000-0001-7717-2765},
D.~~Vieira$^{59}$\lhcborcid{0000-0001-9511-2846},
M.~Vieites~Diaz$^{43}$\lhcborcid{0000-0002-0944-4340},
H.~Viemann$^{70}$,
X.~Vilasis-Cardona$^{75}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{54}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{20}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{13}$\lhcborcid{0000-0002-9283-4541},
F.C.~Volle$^{11}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{10}$\lhcborcid{0000-0001-9905-8031},
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{38}$,
N.~Voropaev$^{38}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{74}$\lhcborcid{0000-0002-4258-4062},
R.~Waldi$^{17}$\lhcborcid{0000-0002-4778-3642},
J.~Walsh$^{29}$\lhcborcid{0000-0002-7235-6976},
C.~Wang$^{17}$\lhcborcid{0000-0002-5909-1379},
J.~Wang$^{5}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{4}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{3}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{67}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{5}$\lhcborcid{0000-0003-4062-710X},
R.~Wang$^{48}$\lhcborcid{0000-0002-2629-4735},
Y.~Wang$^{7}$\lhcborcid{0000-0003-3979-4330},
Z.~Wang$^{44}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{3}$\lhcborcid{0000-0003-0597-4878},
Z.~Wang$^{6}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{50,63}$\lhcborcid{0000-0003-4160-9333},
N.K.~Watson$^{47}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{55}$\lhcborcid{0000-0002-4113-1539},
C.~Weisser$^{58}$,
B.D.C.~Westhenry$^{48}$\lhcborcid{0000-0002-4589-2626},
D.J.~White$^{56}$\lhcborcid{0000-0002-5121-6923},
M.~Whitehead$^{48}$\lhcborcid{0000-0002-2142-3673},
A.R.~Wiederhold$^{50}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{15}$\lhcborcid{0000-0002-4149-4137},
G.~Wilkinson$^{57}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{62}$\lhcborcid{0000-0001-6561-2145},
I.~Williams$^{49}$,
M.~Williams$^{58}$\lhcborcid{0000-0001-8285-3346},
M.R.J.~Williams$^{52}$\lhcborcid{0000-0001-5448-4213},
F.F.~Wilson$^{51}$\lhcborcid{0000-0002-5552-0842},
W.~Wislicki$^{36}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{35}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{17}$\lhcborcid{0000-0001-9178-9921},
G.~Wormser$^{11}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{49}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{62}$\lhcborcid{0000-0002-9337-3476},
K.~Wyllie$^{42}$\lhcborcid{0000-0002-2699-2189},
Z.~Xiang$^{6}$\lhcborcid{0000-0002-9700-3448},
D.~Xiao$^{7}$\lhcborcid{0000-0003-4319-1305},
Y.~Xie$^{7}$\lhcborcid{0000-0001-5012-4069},
A.~Xu$^{5}$\lhcborcid{0000-0002-8521-1688},
J.~Xu$^{6}$\lhcborcid{0000-0001-6950-5865},
L.~Xu$^{3}$\lhcborcid{0000-0003-2800-1438},
M.~Xu$^{50}$\lhcborcid{0000-0001-8885-565X},
Q.~Xu$^{6}$,
Z.~Xu$^{9}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{6}$\lhcborcid{0000-0001-9558-1079},
D.~Yang$^{3}$\lhcborcid{0009-0002-2675-4022},
S.~Yang$^{6}$\lhcborcid{0000-0003-2505-0365},
Y.~Yang$^{6}$\lhcborcid{0000-0002-8917-2620},
Z.~Yang$^{5}$\lhcborcid{0000-0003-2937-9782},
Z.~Yang$^{60}$\lhcborcid{0000-0003-0572-2021},
Y.~Yao$^{62}$,
L.E.~Yeomans$^{54}$\lhcborcid{0000-0002-6737-0511},
H.~Yin$^{7}$\lhcborcid{0000-0001-6977-8257},
J.~Yu$^{65}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{62}$\lhcborcid{0000-0003-0468-3083},
E.~Zaffaroni$^{43}$\lhcborcid{0000-0003-1714-9218},
M.~Zavertyaev$^{16}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{35}$\lhcborcid{0000-0002-1701-9619},
O.~Zenaiev$^{42}$\lhcborcid{0000-0003-3783-6330},
M.~Zeng$^{3}$\lhcborcid{0000-0001-9717-1751},
D.~Zhang$^{7}$\lhcborcid{0000-0002-8826-9113},
L.~Zhang$^{3}$\lhcborcid{0000-0003-2279-8837},
S.~Zhang$^{65}$\lhcborcid{0000-0002-9794-4088},
S.~Zhang$^{5}$\lhcborcid{0000-0002-2385-0767},
Y.~Zhang$^{5}$\lhcborcid{0000-0002-0157-188X},
Y.~Zhang$^{57}$,
A.~Zharkova$^{38}$\lhcborcid{0000-0003-1237-4491},
A.~Zhelezov$^{17}$\lhcborcid{0000-0002-2344-9412},
Y.~Zheng$^{6}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{5}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{6}$\lhcborcid{0009-0005-9485-9477},
Y.~Zhou$^{6}$\lhcborcid{0000-0003-2035-3391},
V.~Zhovkovska$^{11}$\lhcborcid{0000-0002-9812-4508},
X.~Zhu$^{3}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{7}$\lhcborcid{0000-0002-4485-1478},
Z.~Zhu$^{6}$\lhcborcid{0000-0002-9211-3867},
V.~Zhukov$^{14,38}$\lhcborcid{0000-0003-0159-291X},
Q.~Zou$^{4,6}$\lhcborcid{0000-0003-0038-5038},
S.~Zucchelli$^{20,g}$\lhcborcid{0000-0002-2411-1085},
D.~Zuliani$^{28}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{56}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universit{\`a} degli Studi di Padova, Universit{\`a} e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Affiliated with an institute covered by a cooperation agreement with CERN\\
$^{39}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{40}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{41}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{42}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{43}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{44}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{45}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{46}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{47}$University of Birmingham, Birmingham, United Kingdom\\
$^{48}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{49}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{50}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{52}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{53}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{54}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{55}$Imperial College London, London, United Kingdom\\
$^{56}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{57}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{58}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{59}$University of Cincinnati, Cincinnati, OH, United States\\
$^{60}$University of Maryland, College Park, MD, United States\\
$^{61}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{62}$Syracuse University, Syracuse, NY, United States\\
$^{63}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{50}$\\
$^{64}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{65}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{66}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{67}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{68}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{69}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{70}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{17}$\\
$^{71}$Eotvos Lorand University, Budapest, Hungary, associated to $^{42}$\\
$^{72}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{73}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{74}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{75}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{39}$\\
$^{76}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{53}$\\
$^{77}$University of Michigan, Ann Arbor, MI, United States, associated to $^{62}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Central South U., Changsha, China\\
$^{c}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{d}$Excellence Cluster ORIGINS, Munich, Germany\\
$^{e}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{f}$Universit{\`a} di Bari, Bari, Italy\\
$^{g}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{h}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{i}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{j}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{k}$Universit{\`a} di Genova, Genova, Italy\\
$^{l}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{m}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{n}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{o}$Universit{\`a} di Padova, Padova, Italy\\
$^{p}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{q}$Scuola Normale Superiore, Pisa, Italy\\
$^{r}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{s}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{t}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{u}$Universit{\`a} di Siena, Siena, Italy\\
$^{v}$Universit{\`a} di Urbino, Urbino, Italy\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)


